ERASER: Machine Unlearning in MLaaS via an Inference Serving-Aware Approach

Over the past years, Machine Learning-as-a-Service (MLaaS) has received a surging demand for supporting Machine Learning-driven services to offer revolutionized user experience across diverse application areas. MLaaS provides inference service with low inference latency based on an ML model trained using a dataset collected from numerous individual data owners. Recently, for the sake of data owners' privacy and to comply with the "right to be forgotten (RTBF)" as enacted by data protection legislation, many machine unlearning methods have been proposed to remove data owners' data from trained models upon their unlearning requests. However, despite their promising efficiency, almost all existing machine unlearning methods handle unlearning requests independently from inference requests, which unfortunately introduces a new security issue of inference service obsolescence and a privacy vulnerability of undesirable exposure for machine unlearning in MLaaS. In this paper, we propose the ERASER framework for machinE unleaRning in MLaAS via an inferencE seRving-aware approach. ERASER strategically choose appropriate unlearning execution timing to address the inference service obsolescence issue. A novel inference consistency certification mechanism is proposed to avoid the violation of RTBF principle caused by postponed unlearning executions, thereby mitigating the undesirable exposure vulnerability. ERASER offers three groups of design choices to allow for tailor-made variants that best suit the specific environments and preferences of various MLaaS systems. Extensive empirical evaluations across various settings confirm ERASER's effectiveness, e.g., it can effectively save up to 99% of inference latency and 31% of computation overhead over the inference-oblivion baseline.

==> 1.Introduction.tex <==
\section{Introduction}
% no \IEEEPARstart
\label{sec.introduction}
%%\partitle{Background (ML + MLaaS + machine unlearning)}
Machine Learning (ML) has witnessed a meteoric rise in its applications across diverse areas, becoming not only ubiquitous but also essential to enhance user experience \cite{hazelwood2018applied,shaya2010intelligent,bartlett2005recognizing,hauswald2015sirius}. ML-powered applications are oftentimes supported by ML-as-a-Service (MLaaS) \cite{SageMaker2018,Tensorflow2018,Nvidia2020} on the \emph{server} side (e.g., cloud platforms \cite{aws2018,azure2018,cloud2018}), whereby the ML model is built on a large training dataset collected from numerous individuals (i.e., \emph{data owners}) and then deployed to serve inference requests from application users (i.e., \emph{queriers}). 
% The server in MLaaS is responsible for serving requests raised simultaneously by both the queriers and data owners \cite{SageMaker2018,Tensorflow2018,Nvidia2020}.
The server in MLaaS is responsible for handling requests from both queriers and data owners at the same time, with each group having its own unique requirements and concerns.
% , which is a demanding goal since the latter two have distinct and even contradictory desiderata. 
For queriers, the server's primary goal is to provide timely responses to their inference requests, keeping inference latency within an acceptable limit \cite{DBLP:conf/nsdi/CrankshawWZFGS17,DBLP:conf/usenix/ZhangYWY19,DBLP:conf/osdi/GujaratiKAHKVM20,gupta2020deeprecsys,DBLP:conf/usenix/Romero0YK21,gunasekaran2022cocktail}. For data owners, a striking concern is their data privacy, 
which is susceptible to privacy attacks such as black-box membership inference attacks (MIA) \cite{li2021membership,liu2022ml} that can determine if a training sample exists based on inference results.
For server itself, if it is reported that the training model has been contaminated with poisoning data or unauthorized copyrighted contents, prompt deletion is necessary to ensure model security and mitigate legal risks.
% considering the prominent exemplary threat posed by the black-box membership inference attacks \cite{li2021membership,liu2022ml} that determine the existence of a training sample based on inference results. 
% It demands the server to bound the inference latency within an acceptable limit.
 % codified by service-level objectives (SLOs). 
 % Otherwise, the server may turn customers away to a competitor or even risk a penalty, since such delayed inference response can great impact the user experience and even cease to be useful to the querier. 
% For the queriers, a primary goal for the server is to provide timely responses to their inference requests. It demands the server to bound the inference latency within an acceptable limit.
%  % codified by service-level objectives (SLOs). 
%  Otherwise, the server may turn customers away to a competitor or even risk a penalty, since such delayed inference response can great impact the user experience and even cease to be useful to the querier. 

% For the data owners, a striking concern is their data privacy can be under threat, 

% \partitle{Background (Niche)}
Machine unlearning is a nascent research field dedicated to the removal of data and its associated influence from trained ML models in response to unlearning requests, which are typically initiated by data owners based on the RTBF legal principle, and can also be initiated by the server itself, aiming to remove newly identified poisoning data or unauthorized copyrighted data \cite{cao2015towards, guo2019certified, sekhari2021remember, graves2021amnesiac, bourtoule2021machine,DBLP:conf/ndss/WarneckePWR23}. It has gained increasing research attention in recent years, which is mainly prompted by the enforcement of RTBF in data protection regulations worldwide, including the European Union's GDPR \cite{mantelero2013eu}, the Luxembourg's CNPD\cite{CNPD}, and the California Consumer Privacy Act (CCPA) \cite{California2023}.
% , and Canada's proposed Consumer Privacy Protection Act (CPPA) \cite{beardwood2021consumer}.
Most existing researches on machine unlearning focus on improving the efficiency of the machine unlearning mechanism and have achieved promising acceleration over the baseline approach of retraining the ML model on the remaining dataset from scratch \cite{cao2015towards, ginart2019making, brophy2021machine, bourtoule2021machine, ullah2021machine, schelter2021hedgecut, chen2022graph, chen2022recommendation,golatkar2020eternal, wu2020deltagrad, golatkar2020forgetting, nguyen2020variational, neel2021descent, peste2021ssse, golatkar2021mixed, warnecke2021machine, izzo2021approximate, mahadevan2021certifiable}. 
% Among the many existing approaches, SISA (Sharded, Isolated, Sliced, and Aggregated) \cite{bourtoule2021machine} is a prominent example of an exact unlearning solution that is general enough to be applied to various ML models.
Among the many existing approaches, SISA (Sharded, Isolated, Sliced, and Aggregated) \cite{bourtoule2021machine} represents an exact unlearning method that achieves a forgetting effect fully equivalent to retraining from scratch. Unlike other exact unlearning algorithms, which are typically confined to convex learning scenarios \cite{cao2015towards, izzo2021approximate, mahadevan2021certifiable, nguyen2020variational, schelter2021hedgecut, warnecke2021machine} or specific models such as random forests \cite{brophy2021machine} and K-means \cite{ginart2019making}, SISA can be applied across diverse machine learning contexts for exact machine unlearning, including non-convex deep models \cite {chen2022graph, chen2022recommendation}. 
% During the training phase, SISA randomly divides the training dataset into multiple shards, builds a constituent model on each shard, and provides the inference result by aggregating answers from all constituent models. During the unlearning phase, SISA retrains only on the shard that has data to be unlearned to update the corresponding constituent model. 
In addition to efficiency, some work \cite{chen2021machine,marchant2022hard,di2022hidden} have also examined the security and privacy aspects of machine unlearning, revealing that new security and privacy issues can arise. 

% \partitle{Gap}
However, existing machine unlearning approaches mostly focus on the unlearning requests and consider unlearning requests separately from inference requests. This inference-oblivion handling of unlearning requests oversimplifies the problem of machine unlearning in MLaaS and can even conceal potential security and privacy threats in an MLaaS environment where both types of queries exist. 
% Such inference-oblivion consideration over-simplifies the machine unlearning problem and can even conceal potential security and privacy threat for its application in the MLaaS environment where both types of queries exist. 
In fact, as will be detailed in Sec.\ref{sec.definition.and.threat.model}, we have discovered that machine unlearning in MLaaS can suffer from two new security and privacy vulnerabilities if the server uses simple strategies for scheduling unlearning and inference requests. 
% One is the ``unlearning-request-first'' strategy, which has an undiscovered security vulnerability where the server can be indefinitely blocked from responding to normal inference requests. The other is the ``inference-request-first'' strategy, which can incur extra privacy loss for data owners. 
One is the ``unlearning-request-firs'' strategy. Upon receiving unlearning requests, the server temporarily suspends responses to inference requests to prioritize unlearning execution. While this strategy strictly adheres to the RTBF regulatory requirements, it may lead to infinite blocking of responses to normal inference requests. The other is the ``inference-request-first'' strategy. This approach suspends all incoming unlearning requests to prioritize responding to inference requests. Unlearning execution is then postponed until certain conditions are met. 
Alternatively, given adequate resources, another implementation of this strategy is to maintain two parallel systems. Upon receiving an unlearning request, one system continues providing inference services using original model, while the other simultaneously performs the unlearning execution in the background. Once unlearning is complete, a switch between the two systems occurs.
% Alternatively, given adequate resources, two parallel systems can be maintained. Upon receiving an unlearning request, one system continues providing inference services using a model that hasn't undergone unlearning execution, while the other simultaneously performs the unlearning execution in the background. Once unlearning is complete, a switch between the two systems occurs.
These methods persist in utilizing a model that incorporates private data to provide inference services after receiving unlearning requests from data owners, and thus inherently violate the RTBF principle, which mandates that ``personal data must be erased \textbf{immediately} where $\cdots$ withdrawn his consent'' in GDPR \cite{GDPRRightToBeForgotten} and ``this right to erasure also allows you to request the \textbf{immediate} removal of personal data'' in CNPD \cite{CNPDDroitOubli}. Adopting an ``inference-request-first'' exposes users’ data to potential threats like MIA even when data deletion has already been requested, thereby escalating privacy risks for data owners.
% However, such method inherently violates the RTBF principle. After receiving an unlearning request from a data owner, the server continues to use a model containing the data owner's information to provide inference services, thereby exposing it to potential threats like MIA even when data deletion has already been requested, leading to increased privacy risks for data owners.
If an unlearning request is intended to remove poisoning data, then the harm caused by the poisoning data will persist, and the potential ``landmines'' it poses can be triggered at any time during the suspension. If the unlearning request aims to delete copyrighted data, the losses from copyright infringement will continue to accumulate during the suspension, putting additional compensation pressure on the server.
Both strategies are implicitly suggested by existing machine unlearning works and proposed in an inference-oblivion manner.

% In this paper, we propose \projectname: machin\underline{\textbf{E}} unlea\underline{\textbf{R}}ning in MLa\underline{\textbf{AS}} via an inferenc\underline{\textbf{E}} se\underline{\textbf{R}}ving-aware approach. Our main contributions are as follows.
To address the issues mentioned above, we propose \projectname: machin\underline{\textbf{E}} unlea\underline{\textbf{R}}ning in MLa\underline{\textbf{AS}} via an inferenc\underline{\textbf{E}} se\underline{\textbf{R}}ving-aware approach. \projectname ~can reduce inference latency by conditionally postponing unlearning execution through a certified inference consistency mechanism.
The method for determining whether postponing unlearning execution as in the second simple strategy will incur extra risks involves distinguishing whether the model's response to an inference request after unlearning execution differs from that of a model retaining the sensitive data.
% This is because such discrepancies indicate that the sensitive data has a significant impact on the model, making it extremely susceptible to MIA that can potentially identify the data.
The discrepancy would indicate that the sensitive data has a significant impact on the model's response to this inference request.
% The reason why postponing unlearning execution would incur privacy risks in the second simple strategy is that the model's response to an inference request after unlearning execution may differ from that of a model retaining the sensitive data. Such discrepancies indicate that the sensitive data has a significant impact on the model, making it more susceptible to MIA that can potentially identify the data.
Unlearning execution can only be postponed when it's ensured that the server's response to inference requests remains consistent before and after the unlearning execution. However, verifying this consistency by directly executing the unlearning process is meaningless. Therefore, we exploit the inherent structural characteristics of SISA to design a certified inference consistency mechanism. This mechanism can anticipate whether the prediction outcome would change after unlearning execution. If deemed consistent, denoting certified prediction consistency, the unlearning execution can be postponed, allowing for an immediate response to the current inference request. All postponed unlearning executions can be batch-processed, thereby reducing processing time and computational resource consumption without introducing additional privacy risks, ultimately enhancing the response speed to inference requests.

% Considering the diverse resources and preferences of different MLaaS servers, we offer three groups of design options under the ERASER framework: the capability to simultaneously maintain both training and inference environments, the timing for executing unlearning execution, and the handling strategy for inference requests that cannot achieve consistency. Based on these options, we have designed seven distinct methods. Servers can choose the appropriate method based on their preferences regarding response speed, resource consumption, and privacy protection.

Although this framework appears intuitively applicable, the diversity in server types, alongside significant disparities in their service objectives and available resources, presents many challenges in practical deployment. To address these challenges, we investigate existing MLaaS solutions and identified three core options that impact our framework's deployment: the ability to concurrently manage both training and inference environments, the timing of unlearning execution, and the strategy for handling inference requests that fail to achieve consistency. Based on these options, we have developed seven distinct methods. Servers can select the most suitable method according to their preferences for response speed, resource consumption, and privacy protection.
% \partitle{Method (Variations)}

% \partitle{Experiments}

% \partitle{Summary+contributions}

\begin{itemize}[leftmargin=*]
  % \item To the best of our knowledge, we are the first to study machine unlearning in the MLaaS setting and examine the security and privacy consequence of serving inference requests and unlearning requests at the same time. In particular, we have identified two new security and privacy vulnerabilities in this unlearning setting, resulting from two simplified strategies suggested by existing inference-oblivion machine unlearning works.
  \item To the best of our knowledge, we are the first to identify the security and privacy vulnerabilities of machine unlearning in the MLaaS setting, resulting from two simplified strategies suggested by existing inference-oblivion machine unlearning works.
  % \item We propose \projectname, a new machine unlearning framework for MLaaS developed in an inference serving-aware manner, which can reduce inference latency while avoiding the two security and privacy vulnerabilities. The key is the development of a certified prediction consistency mechanism that allows inference requests to be executed without waiting for the execution of pending unlearning requests.
  \item We propose \projectname, a new machine unlearning framework for MLaaS developed in an inference serving-aware manner, which can reduce inference latency while avoiding security and privacy vulnerabilities.
  \item We further propose seven variants under \projectname ~based on three design options, each being tailored to specific environments and preferences of different MLaaS systems.
  % \item We perform a comprehensive evaluation on XX machine learning models using XX real-world datasets to examine the performance of \projectname ~under XX different affecting factors, including the distributions of the inference and unlearning requests XXX. The results demonstrate that \projectname ~and its variants under different options greatly reduce the inference latency over the inference-oblivious baselines in different settings, achieving XX\% to XX\% inference latency saving. 
  \item We perform a comprehensive evaluation on four machine learning models using four real-world datasets to assess the performance of \projectname. 
  % We consider different settings by taking into account  varying factors, including the distributions and density of the inference and unlearning requests, server computing capability, and hyper-parameter settings in \projectname. 
  The results demonstrate that \projectname ~and its variants significantly reduce inference latency and computational overhead compared to the inference-oblivious baseline in different settings, achieving up to 99\% saving in inference latency  and 31\% saving in computation overhead. 
  % We perform a comprehensive evaluation on four machine learning models using four real-world datasets to examine the performance of \projectname ~under various different affecting factors, including the distributions and density of the inference and unlearning requests, server computing capability, and hyper-parameters settings in \projectname. The results demonstrate that \projectname ~and its variants under different options greatly reduce the inference latency over the inference-oblivious baselines in different settings, achieving 99\% inference latency saving and 31\% computation overhead saving at most. 
\end{itemize}

% \partitle{Roadmap}
% Section \ref{sec.background} introduces background and preliminary. Section \ref{sec.definition.and.threat.model} defines the threat model and presents two motivating attacks. Section \ref{sec.framework} proposes the \projectname ~framework. Section \ref{sec.variants} explores design options in the \projectname ~framework targeting different MLaaS environments. Section \ref{sec.experiment} presents the empirical evaluation results and analysis.
% % Section \ref{sec.conclusion} discusses more related works. 
% Section \ref{sec.conclusion} draws a conclusion of the paper and discusses future works. Additionally, Appendix A-D contains more theoretical results; Appendix E-F provides more content about algorithm design; Appendix G-H presents more experiment results. 

\begin{figure*}[t]
	\centering
	\includegraphics[width=0.95\textwidth]{figure/Scheme_v3.pdf}
	\caption{Illustration of comparison between \projectname ~and SISA with two inference-oblivion strategies. Green represents inference service without privacy risk, red indicates inference with privacy risk, and yellow signifies unlearning execution. \textbf{IR}: \textbf{I}nference \textbf{R}equest; \textbf{UR}: \textbf{U}nlearning \textbf{R}equest.}
	\label{fig: scheme}
	% \vspace{-2em}
\end{figure*}

==> nwz/abstrac_outline.tex <==
\begin{abstract}
    Over the past few years, Machine Learning-as-a-Service (MLaaS) has received a surging demand for supporting Machine Learning-driven services to offer revolutionized user experience across diverse application areas. MLaaS provides inference service with low inference latency to application users based on an ML model trained using a dataset collected from numerous individual data owners. Recently, for the sake of data owners' privacy and to comply with the ``right to be forgotten (RTBF)'' as enacted by data protection legislation, many machine unlearning methods have been proposed to remove data owners' data from trained models upon their unlearning requests. However, despite their promising efficiency, almost all existing machine unlearning methods handle unlearning requests separately form inference requests.
    Naively applying existing methods in MLaaS setting may introduce a security issue of service obsolescence and a privacy issue of undesirable exposure. The former refers to a significant slowdown in MLaaS service latency, making the service obsoleted in the competitive market. The later refers to the delay in processing unlearning requests, violating the RTBF regulation and expose private data to attacks like membership inference attack.

    In this paper, we propose the \projectname ~framework for machin\underline{E} unlea\underline{R}ning in MLa\underline{AS} via an inferenc\underline{E} se\underline{R}ving-aware approach. 
    \projectname ~strategically choose appropriate unlearning execution timing to address the service obsolescence issue. A novel inference consistency certification mechanism is proposed to avoid the violation of RTBF principle caused by postponed unlearning execution, and thus address the undesirable exposure issue.
    \projectname ~offers three groups of design choices to allow for tailor-made variants that best suit the specific environments and preferences of various MLaaS systems. 
    Extensive empirical evaluations across various settings confirm \projectname's effectiveness, e.g., it can effectively save up to 99\% of inference latency and 31\% of computation overhead over the inference-oblivion baseline.
\end{abstract}

==> nwz/abstract.tex <==
\begin{abstract}
    Machine Learning-as-a-Service (MLaaS) is a popular technology that provides fast inference services using models trained on data from multiple sources. However, MLaaS faces regulatory pressures related to data security and privacy, like the ``right to be forgotten (RTBF)''. Unlearning methods are a well-known approach to comply with data protection laws, but existing methods do not consider inference requests in MLaaS scenarios. Designing an unlearning method for MLaaS is challenging, as naively applying existing methods may cause the security issue of service obsolescence and the privacy threat of undesirable exposure. Service obsolescence issue refers to a significant slowdown in MLaaS service response time, making the service obsolete and non-viable in the competitive market. Undesirable exposure risk refers to a delay in processing unlearning requests, violating the RTBF regulatory and releasing privacy data that unlearning requests want to remove.

    To solve the two issues, in this paper, we propose a framework named \projectname. \projectname ~predicts the impact of an unlearning request $u$ on an inference request $q$, and decides the execution of $u$ based on the prediction result.
    Specifically, when $u$ may affect the response to $q$, ERASER first executes $u$ and then responds to $q$. We theoretically prove that ERASER does not have the Eraser Delay Hazard issue. When $q$ does not affect the response to $u$, ERASER temporarily postpones the execution of $u$ and will execute a batch of unlearning requests together in the future. We theoretically prove that ERASER does not have the Service Obsolescence Threat issue. Due to the different environments of various MLaaS systems, it is challenging to implement ERASER in a way that best fits an MLaaS system. In this paper, we offer three groups of design choices to allow for tailor-made variants that best suit MLaaS systems. Extensive empirical evaluations across various settings confirm \projectname's effectiveness, e.g., it can effectively save up to 99\% of inference latency and 31\% of computation overhead over the inference-oblivion baseline.
\end{abstract}

==> nwz/introduction.tex <==
\section{Introduction}
\label{sec.introduction}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.47\textwidth]{figure/MLaaS.pdf}
	\caption{Scheme of MLaaS}
	\label{fig: mlaas}
\end{figure}

\begin{figure*}[t]
	\centering
	\includegraphics[width=0.95\textwidth]{figure/Scheme_v3.pdf}
	\caption{Comparison between \projectname ~and naive strategies. Green represents inference without privacy risk, red indicates inference with privacy risk, and yellow signifies unlearning execution. \textbf{IR}: \textbf{I}nference \textbf{R}equest; \textbf{UR}: \textbf{U}nlearning \textbf{R}equest.}
	\label{fig: scheme}
	% \vspace{-2em}
\end{figure*}

With the rise of machine learning~\cite{hazelwood2018applied,shaya2010intelligent,bartlett2005recognizing,hauswald2015sirius}, there has been an increasing focus on data security and privacy, leading to the introduction of numerous laws and regulations (e.g., RTBF~\cite{mantelero2013eu} and the California Consumer Privacy Act (CCPA) \cite{California2023}). As a promising approach for complying with these data protection laws, machine unlearning has garnered growing research interest in recent years~\cite{cao2015towards, guo2019certified, sekhari2021remember, graves2021amnesiac, bourtoule2021machine,DBLP:conf/ndss/WarneckePWR23}. Machine unlearning methods are capable of eliminating data and its associated influence from trained machine learning models.

%写：Existing unlearning methods focus on the scenario where XXXX. However, recently, a new paradigm called MLaaS emerges, which not only executes data owners' unlearning requests but also answer users' inference requests. Specifically, as depicted in Figure~\ref{fig: mlaas}, 在MLaaS系统中有哪些角色，每个角色分别干什么，是怎么干的。MLaaS system的特点是（1）需要及时响应以及（2）需要保持一致。

Existing unlearning methods are primarily designed for scenarios where the demand to ``be forgotten" is addressed in a manner that is separate from the requirements of model inference.
However, recent ML-powered applications are oftentimes supported by ML-as-a-Service (MLaaS) \cite{SageMaker2018,Tensorflow2018,Nvidia2020} on the \emph{server} side (e.g., cloud platforms \cite{aws2018,azure2018,cloud2018}), whereby the ML model is built on a large training dataset collected from numerous individuals (i.e., \emph{data owners}) and then deployed to serve inference requests from application users (i.e., \emph{queriers}) as depicted in Figure \ref{fig: mlaas}. The server in MLaaS is responsible for handling requests from both queriers and data owners at the same time.
For queriers, the server's primary goal is to provide timely responses to their inference requests, keeping inference latency within the bounds of service-level objectives (SLOs). \cite{DBLP:conf/nsdi/CrankshawWZFGS17,DBLP:conf/usenix/ZhangYWY19,DBLP:conf/osdi/GujaratiKAHKVM20,gupta2020deeprecsys,DBLP:conf/usenix/Romero0YK21,gunasekaran2022cocktail}. Failure to maintain an acceptable latency could result in clients turning to competitors or incurring penalties.
For data owners, a striking concern is their data privacy, which is susceptible to privacy attacks such as black-box membership inference attacks (MIA) \cite{li2021membership,liu2022ml} that can determine if a training sample exists based on inference results.
Besides, if the server discover that the training model has been compromised by poisoning data or unauthorized copyrighted content, prompt action for data erasure is also imperative to ensure model security and to mitigate legal risks.

%写：由于现有的unlearning methods并没有考虑MLaaS的这些特点，所以我们无法简单地将现有unlearning methods使用在MLaaS系统里。
However, existing machine unlearning approaches mostly treat unlearning requests independent from inference requests. This inference-oblivious characteristic precludes the straightforward implementation in the MLaaS scenarios. 
As will be detailed in Sec.\ref{sec.definition.and.threat.model}, we observe that if servers adopt the naive strategies for scheduling unlearning and inference requests, it can lead to the security issue of service obsolescence and the privacy issue of undesirable exposure.
%写两句话定义一下什么是service obsolescence和undesirable exposure
The former refers to a significant slowdown in MLaaS service latency, making the service obsolete in the competitive market. The later refers to a delay in processing unlearning requests, violating the RTBF regulation and expose private data to attacks like MIA.
One such naive approach is the "unlearning-request-first" strategy, depicted in the top row of Figure \ref{fig: scheme}. Upon receiving unlearning requests, the server temporarily suspends processing inference requests to prioritize unlearning. While this method rigorously complies with the RTBF regulatory mandates, it could result in intolerable response latency, leading to service obsolescence. Conversely, the "inference-request-first" strategy, illustrated in the middle row of Figure \ref{fig: scheme}, involves suspending all unlearning requests to prioritize inference requests. Unlearning is deferred until certain conditions (e.g., number of the pending unlearning requests ) %写(：e.g., ) 
are met. 
%写这个variant感觉太长了，导致这一段太长。而且两个策略讲完又加了一个variant，会confuse。是否可以不写？如果一定要写的话，是否可以考虑改成一句话简单带过，比如说使用两套系统进行切换由于回答的那套系统没有使用更新后的模型也归类为“inference-request-first”策略。尽量避免指向不明的the、it、this之类的代词。
% Another variant of the "inference-request-first" strategy, given sufficient resources, involves maintaining two parallel systems. When an unlearning request is received, one system continues to offer inference services using the original model, while the other concurrently executes the unlearning process in the background. The switch to the updated system occurs post unlearning completion. 
Another variant of the "inference-request-first" strategy is to process the unlearning requests in the back end rather than suspending them while offering inference services with the original model.
%写：由于inference-request-first 策略没有及时使用更新的模型响应inference request,可能会产生XXX问题。比如说，举个XXX问题的具体实例。
Both variants of the second strategy persist in using a model containing data that need deletion to provide inference services even after receiving unlearning requests. This practice inherently breaches the RTBF principle, which mandates ``\textbf{immediately erasure}'' \cite{GDPRRightToBeForgotten, CNPDDroitOubli}. Adopting an ``inference-request-first" strategy exposes users’ data to potential threats like MIA even when data deletion has already been requested, leading to undesirable exposure privacy risk.
% If an unlearning request is intended to remove poisoning data, then the harm caused by the poisoning data will persist, and the potential ``landmines" it poses can be triggered at any time during the suspension. If the unlearning request aims to delete copyrighted data, the losses from copyright infringement will continue to accumulate during the suspension, putting additional compensation pressure on the server.

To address the issues mentioned above, we propose \projectname: machin\underline{\textbf{E}} unlea\underline{\textbf{R}}ning in MLa\underline{\textbf{AS}} via an inferenc\underline{\textbf{E}} se\underline{\textbf{R}}ving-aware approach. \projectname ~can mitigating the issue of obsolescence by strategically postponing unlearning execution through a certified inference consistency mechanism.
The underlying cause of the privacy risk associated with postponing unlearning execution stems from the fact that the presence or absence of certain training data may lead to different responses for the same inference request. This discrepancy can be exploit by the attackers. If the model's response to a current inference request remains consistent before and after the erasure of these data, it becomes feasible to postpone the unlearning execution. However, the prerequisite for verifying consistency is to execute unlearning to obtain the current response, which paradoxically contradicts our goal of deferring unlearning. This scenario is akin to needing a key to unlock a door, but the key itself is locked behind that very door.
To overcome this conundrum, we leverage the inherent structural characteristics of SISA to devise a inference consistency certification mechanism. This mechanism enables us to predict whether the response would change after unlearning execution. If deemed consistent, the unlearning execution can be postponed, allowing for an immediate response to the inference request.  All deferred unlearning requests can then be batch-processed, significantly reducing processing time and computational overhead without introducing additional privacy risks.

Although this framework appears intuitively applicable, the diversity in server types, alongside significant disparities in their service objectives and available resources, presents many challenges in practical deployment. To address these challenges, we investigate existing MLaaS solutions and identified three core options that impact our framework's deployment: the ability to concurrently manage both training and inference environments, the timing of unlearning execution, and the strategy for handling inference requests that fail to achieve consistency. Based on these options, we have developed seven distinct methods. Servers can select the most suitable method according to their preferences for response speed, resource consumption, and privacy protection.
% \partitle{Method (Variations)}

% \partitle{Experiments}

% \partitle{Summary+contributions}

\begin{itemize}[leftmargin=*]
  % \item To the best of our knowledge, we are the first to study machine unlearning in the MLaaS setting and examine the security and privacy consequence of serving inference requests and unlearning requests at the same time. In particular, we have identified two new security and privacy vulnerabilities in this unlearning setting, resulting from two simplified strategies suggested by existing inference-oblivion machine unlearning works.
  \item To the best of our knowledge, we are the first to identify the security and privacy vulnerabilities of machine unlearning in the MLaaS setting, resulting from two simplified strategies suggested by existing inference-oblivion machine unlearning works.
  % \item We propose \projectname, a new machine unlearning framework for MLaaS developed in an inference serving-aware manner, which can reduce inference latency while avoiding the two security and privacy vulnerabilities. The key is the development of a certified prediction consistency mechanism that allows inference requests to be executed without waiting for the execution of pending unlearning requests.
  \item We propose \projectname, a new machine unlearning framework for MLaaS developed in an inference serving-aware manner, which can reduce inference latency while avoiding security and privacy vulnerabilities.
  \item We further propose seven variants under \projectname ~based on three design options, each being tailored to specific environments and preferences of different MLaaS systems.
  % \item We perform a comprehensive evaluation on XX machine learning models using XX real-world datasets to examine the performance of \projectname ~under XX different affecting factors, including the distributions of the inference and unlearning requests XXX. The results demonstrate that \projectname ~and its variants under different options greatly reduce the inference latency over the inference-oblivious baselines in different settings, achieving XX\% to XX\% inference latency saving. 
  \item We perform a comprehensive evaluation on four machine learning models using four real-world datasets to assess the performance of \projectname. 
  % We consider different settings by taking into account  varying factors, including the distributions and density of the inference and unlearning requests, server computing capability, and hyper-parameter settings in \projectname. 
  The results demonstrate that \projectname ~and its variants significantly reduce inference latency and computational overhead compared to the inference-oblivious baseline in different settings, achieving up to 99\% saving in inference latency  and 31\% saving in computation overhead. 
  % We perform a comprehensive evaluation on four machine learning models using four real-world datasets to examine the performance of \projectname ~under various different affecting factors, including the distributions and density of the inference and unlearning requests, server computing capability, and hyper-parameters settings in \projectname. The results demonstrate that \projectname ~and its variants under different options greatly reduce the inference latency over the inference-oblivious baselines in different settings, achieving 99\% inference latency saving and 31\% computation overhead saving at most. 
\end{itemize}
